Curve Your Attention: Mixed-Curvature Transformers for Graph Representation Learning

Real-world graphs naturally exhibit hierarchical or cyclical structures that are unfit for the typical Euclidean space. While there exist graph neural networks that leverage hyperbolic or spherical spaces to learn representations that embed such structures more accurately, these methods are confined under the message-passing paradigm, making the models vulnerable against side-effects such as oversmoothing and oversquashing. More recent work have proposed global attention-based graph Transformers that can easily model long-range interactions, but their extensions towards non-Euclidean geometry are yet unexplored. To bridge this gap, we propose Fully Product-Stereographic Transformer, a generalization of Transformers towards operating entirely on the product of constant curvature spaces. When combined with tokenized graph Transformers, our model can learn the curvature appropriate for the input graph in an end-to-end fashion, without the need of additional tuning on different curvature initializations. We also provide a kernelized approach to non-Euclidean attention, which enables our model to run in time and memory cost linear to the number of nodes and edges while respecting the underlying geometry. Experiments on graph reconstruction and node classification demonstrate the benefits of generalizing Transformers to the non-Euclidean domain.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/8_analysis.tex <==
\input{tables/transductive_dataset_statistics}


\begin{equation}
    \underbrace{\frac{1}{\sqrt{n}}Q G K^T V}_{\text{Euclidean Representations}} \Longleftrightarrow \underbrace{\mathbb{G}(Q, K)V}_{\text{Riemannian Representations}}
\end{equation}

\paragraph{Tensors.}

\begin{definition}(Tensor Representation of Transformer). Let us denote $V \coloneqq v^i  \partial_i$, $Q \coloneqq n^{-\frac{1}{4}} q^i \partial_i$, $K \coloneqq n^{-\frac{1}{4}} k^i \partial_i$ be latent information represented as tensor fields on tangent space $T \mathcal{M}$ of $d$-dimensional smooth manifolds $\mathcal{M}$. We call $\mathbb{G} \in \mathcal{T}^2(T^{*}\mathcal{M})$ a geometric aggregator, which is a $2$-tensor taking query and key tensors ($\ie K, Q$). Then, 
\begin{equation}
    \mathbb{G}[P(Q), K]V \coloneqq \frac{1}{\sqrt{n}}g_{ij} q^i k^j (v^k\partial_k) \in \mathcal{X}(\mathcal{M}, T\mathcal{M})
\end{equation}
\end{definition}
In local coordinates, the above definition is specified as
\begin{equation}
\begin{split}
     \mathbb{G}(P_y^x Q_{y}, K_{x})V_{x} &= \mathbb{G}\left(n^{-\frac{1}{4}} P_y^x(q^i_y \partial_i^{y}), n^{-\frac{1}{4}}k^j_x \partial_j^x \right)V_x 
     \\ & = \frac{1}{\sqrt{n}}g_{ij}|_{x}(dx_i \otimes dx_j)( P_y^x (q^i_y) \partial_i^x, k^j \partial_j^x)(v^k_x \partial_k^x)
     \\ & = \frac{1}{\sqrt{n}} \sum_{i, j}^{d} g_{ij}|_x (P_y^x q^i_y) k^j_x \left( \sum_k^d v^k_x \partial_k^x \right)
\end{split}
\end{equation}
Let us assume that $\{ \partial_i^y \}_{i \in \{1, \cdots, d\}} \coloneqq \boldsymbol{\partial}^y$ spans $T_y \mathcal{M}$. Then, by isometry of parallel transport, the last equality holds as $P_y^x \boldsymbol{\partial}^y \coloneqq \boldsymbol{\partial}^x$ is a base of $T_x \mathcal{M}$.
\begin{itemize}
    \item \textit{Symmetrization.} If we consider the symmetrization of tensor 
    \begin{equation}
        \mathbf{Sym}^2(T^{*}\mathcal{M}) \subset \mathcal{T}^2(T^{*}\mathcal{M})
    \end{equation}

\end{itemize}



\paragraph{Parallel Transport.} Let $\gamma(t)$ be a geodesic with terminal constraints $\gamma(0) = x$ and $\gamma(1) = y$. 


\paragraph{Solving Geodesic Equation.}
terminal state constraints: Interpolation
initial state constraints: Extrapolation

\begin{equation}
    \ddot{T}^i + \Gamma_{jk}^{i}\dot{T}^j \dot{T}^k = 0, \quad T(0) = P, \dot{T}(0) = \mathbb{G}(Q, K)V
\end{equation}


==> sections/9_rebuttal.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=.45\textwidth]{figures/runtime_vs_tokengt.pdf}
    \vspace{-5pt}
    \caption{Runtime comparison of FPS-T vs. TokenGT on graphs with increasing number of nodes and edges. The x-axis shows the total number of nodes and edges (in $10^7$). The \textcolor{c0}{blue solid line (left y-axis)} shows the absolute runtime of FPS-T, and the \textcolor{c2}{green dashed line (right y-axis)} shows its ratio relative to TokenGT. FPS-T runs in asymptotic cost linear to the number of nodes and edges due to linearized attention (Section 4.5). The runtime ratio vs. TokenGT converges towards 1, indicating that the additional cost of Riemannian operations on top of TokenGT is dominated on large networks.}
    \vspace{-10pt}
\end{figure}

\begin{figure}[!h]
    \centering
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/GR_pareto_web-edu.pdf}
        \vspace{-15pt}
        \caption{Web-Edu}
    \end{subfigure}
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/GR_pareto_power.pdf}
        \vspace{-15pt}
        \caption{Power}
    \end{subfigure}
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/GR_pareto_facebook.pdf}
        \vspace{-15pt}
        \caption{Facebook}
    \end{subfigure}
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/GR_pareto_bio-wormnet.pdf}
        \vspace{-15pt}
        \caption{Bio-Worm}
    \end{subfigure}
    \vspace{-10pt}
    \caption{Model size (x-axis) vs. mAP score (y-axis) plots of FPS-T and TokenGT from each graph reconstruction task. The blue-shade indicates the pareto-efficiency gap between TokenGT and FPS-T in terms of model size. FPS-T is consistently more pareto-efficient than TokenGT across all datasets, with Web-Edu showing the largest gap due to its mixed-geometry deviating the most from Euclidean.}
    \vspace{-10pt}
\end{figure}

\begin{figure}[!h]
    \centering
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=.6\textwidth]{figures/tree.jpg}
        \caption{Tree}
    \end{subfigure}
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=.6\textwidth]{figures/sphere.jpg}
        \caption{Sphere}
    \end{subfigure}
    \begin{subfigure}{0.245\textwidth}
        \centering
        \raisebox{3pt}{\includegraphics[width=.8\textwidth]{figures/torus.jpg}}
        \caption{Torus}
    \end{subfigure}
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=.6\textwidth]{figures/ring_of_trees.jpg}
        \caption{Ring of Trees}
    \end{subfigure}
    \vspace{-10pt}
    \caption{Example illustrations of geometric graphs used in our synthetic experiment. For Tree, we use a uniform tree with depth 5 and branching factor 4. For Sphere, we randomly sample 2000 nodes from a unit sphere, and connect two nodes with a edge if they are within a spherical distance of 0.3. Similarly for Torus, we randomly sample 2000 nodes and connect two nodes if they are within a toroidal distance of 0.02. For Ring of Trees, we attach trees with 4 branches on a cycle with 10 nodes.}
    \vspace{-15pt}
\end{figure}

\input{tables/rebuttal_synthetic}

==> tables/LRA.tex <==
\begin{table}[!ht]
    \centering
    \caption{Experiments on sequence classification on LRA. Numbers in parentheses denote input sequence length} \label{tab:LRA_experiments} 
    \vspace{.1in}
    \resizebox{\textwidth}{!}{\begin{tabular}{l|ccccc}
        \toprule
        Method & ListOps (1K) & Text (4K) & Retrieval (4K) & Image (1K) & Pathfinder (1K)\\
        \midrule
        Vanilla &  &  &  &  &  \\
        Linearized &  &  &  &  &  \\
        Linear &  &  &  &  &  \\
        Performer &  &  &  &  &  \\
        Reformer &  &  &  &  &  \\
        Nystromformer &  &  &  &  &  \\
        Ours &  &  &  &  &  \\
        \bottomrule
    \end{tabular}
    }
\end{table}



==> tables/ablation.tex <==
\begin{table}[!ht]
    \centering
    \caption{Ablation study by replacing each component in Transformer to its Euclidean counterpart.} \label{tab:ablation_experiments} 
    \vspace{.1in}
    \resizebox{\textwidth}{!}{\begin{tabular}{l|cccc|cc}
        \toprule
        Case & PT? & st-MHA? & st-FFN? & st-Embed/Decode? & NC & LP\\
        \midrule
        Ours & \cmark & \cmark & \cmark & \cmark & 0.00$\pm$0.00 & 0.00$\pm$0.00\\
        Case 1 & \xmark & \cmark & \cmark & \cmark & 0.00$\pm$0.00 & 0.00$\pm$0.00\\
        Case 2 & \xmark & \xmark & \cmark & \cmark & 0.00$\pm$0.00 & 0.00$\pm$0.00\\
        Case 3 & \xmark & \xmark & \xmark & \cmark & 0.00$\pm$0.00 & 0.00$\pm$0.00\\
        TokenGT & \xmark & \xmark & \xmark & \xmark & 0.00$\pm$0.00 & 0.00$\pm$0.00\\
        \bottomrule
    \end{tabular}
    }
\end{table}



==> tables/graph_experiments.tex <==
\begin{table}[!ht]
    \centering
    \caption{Node classification (in F1) and link prediction (in ROC-AUC) results. We categorize methods that are Euclidean-based, those that operate on the hyperbolic space, a combination of different curvatures, and our method.} \label{tab:graph_experiments} 
    \vspace{.1in}
    \resizebox{\textwidth}{!}{\begin{tabular}{l|cc|cc|cc|cc}
        \toprule
        Dataset & \multicolumn{2}{c|}{Airport} & \multicolumn{2}{c|}{Pubmed} & \multicolumn{2}{c|}{Cora} & \multicolumn{2}{c}{Citeseer} \\
        $\delta$-hyperbolicity & \multicolumn{2}{c|}{1.0} & \multicolumn{2}{c|}{3.5} & \multicolumn{2}{c|}{4.5} & \multicolumn{2}{c}{11.0} \\
        \midrule
        Task & NC & LP & NC & LP & NC & LP & NC & LP\\
        \midrule
        \textsc{GCN} & 00.00$\pm$0.00 & 00.00$\pm$0.00 & 00.00$\pm$0.00 & 00.00$\pm$0.00 & 00.00$\pm$0.00 & 00.00$\pm$0.00 & 00.00$\pm$0.00 & 00.00$\pm$0.00 \\
        \textsc{GAT} &  &  &  &  &  &  &  &  \\
        \textsc{SAGE} &  &  &  &  &  &  &  &  \\
        \textsc{SGC} &  &  &  &  &  &  &  &  \\
        \textsc{TokenGT} &  &  &  &  &  &  &  &  \\
        \midrule
        \textsc{HGCN} &  &  &  &  &  &  &  &  \\
        \textsc{HGNN} &  &  &  &  &  &  &  &  \\
        \textsc{HGAT} &  &  &  &  &  &  &  &  \\
        \textsc{GIL} &  &  &  &  &  &  &  &  \\
        \midrule
        \textsc{$\kappa$-GCN ($\mathbb{H}^{16}$)} &  &  &  &  &  &  &  &  \\
        \textsc{$\kappa$-GCN ($\mathbb{S}^{16}$)} &  &  &  &  &  &  &  &  \\
        \textsc{$\kappa$-GCN ($\mathbb{H}^{8} \times \mathbb{S}^{8}$)} &  &  &  &  &  &  &  &  \\
        \textsc{$\mathcal{Q}$-GCN} &  &  &  &  &  &  &  &  \\
        \midrule
        \textsc{(Ours)} &  &  &  &  &  &  &  &  \\
        \bottomrule
    \end{tabular}
    }
\end{table}



==> tables/inductive_dataset_statistics.tex <==
\begin{table}[!ht]
    \centering
    \caption{Dataset statistics for molecular property prediction tasks.} \label{tab:inductive_dataset_statistics} 
    \vspace{.1in}
    \resizebox{.9\textwidth}{!}{\begin{tabular}{l|ccc|ccccccc}
        \toprule
        Task & \multicolumn{3}{c|}{Regression} & \multicolumn{7}{c}{Binary Classification}\\
        Dataset & ESOL & FREESOLV & LIPO & BACE & BBBP & CLINTOX & HIV & SIDER & TOX21 & TOXCAST \\
        \midrule
        \# molecules & 1,128 & 642 & 4,200 & 1,513 & 2,039 & 1,477 & 41,127 & 1,427 & 7,831 & 8,576 \\
        Avg. \# atoms & 13.3 & 8.7 & 27.0 & 34.1 & 24.1 & 26.2 & 25.5 & 33.6 & 18.6 & 18.8 \\
        Avg. \# bonds &  13.7 & 8.4 & 29.5 & 36.9 & 26.0 & 27.9 & 27.5 & 35.4 & 19.3 & 19.3 \\
        \# elements & 9 & 9 & 12 & 8 & 13 & 28 & 55 & 40 & 51 & 53 \\
        \# targets & 1 & 1 & 1 & 1 & 1 & 2 & 1 & 27 & 12 & 617\\
        \bottomrule
    \end{tabular}
    }
\end{table}



==> tables/link_prediction.tex <==
\begin{table}[!t]
    \centering
    \caption{Link Prediction results in ROC-AUC scores.\sungjun{Likely that we will drop LP.}} \label{tab:link_prediction} 
    \vspace{.1in}
    \resizebox{\textwidth}{!}{\begin{tabular}{l|cccc|cccc}
        \toprule
        Dataset & Texas & Cornell & Wisconsin & Actor & Airport & Citeseer & Pubmed & Cora \\
        $\mathcal{H}(G)$ & 0.11 & 0.13 & 0.20 & 0.22 & 0.72 & 0.74 & 0.80 & 0.81\\
        \midrule
        \textsc{MLP} &  &  &  &  &  &  &  & \\
        \textsc{GCN} &  &  &  &  &  &  &  & 92.89{\scriptsize $\pm$0.12} \\
        \textsc{GAT} &  &  &  &  &  &  &  & \\
        \textsc{SAGE} &  &  &  &  &  &  & 95.41{\scriptsize $\pm$0.08} & \\
        \textsc{SGC} &  &  &  &  &  &  &  & \\
        \textsc{TokenGT} &  & 68.52{\scriptsize $\pm$1.63} &  & 71.80{\scriptsize $\pm$0.31} & 94.54{\scriptsize $\pm$0.34} & 97.01{\scriptsize $\pm$0.22} & 96.70{\scriptsize $\pm$0.06} & 92.90{\scriptsize $\pm$0.46} \\
        \midrule
        \textsc{HGCN} &  &  &  &  &  &  &  & \\
        \textsc{HGNN} &  &  &  &  &  &  &  & \\
        \textsc{HAT} &  &  &  &  &  &  &  & \\
        \midrule
        \textsc{$\kappa$-GCN} &  &  &  &  &  &  &  & \\
        \textsc{$\mathcal{Q}$-GCN} &  &  &  &  &  &  &  & \\
        \midrule
        \textsc{\modelname{}} & 75.02{\scriptsize $\pm$1.60} & 67.76{\scriptsize $\pm$1.81} & 80.52{\scriptsize $\pm$1.49} & 72.54{\scriptsize $\pm$0.33} &  &  &  & \\
        \bottomrule
    \end{tabular}
    }
\end{table}



==> tables/molecular_property_prediction.tex <==
\begin{table}[!ht]
    \centering
    \caption{Molecular Property Prediction results.} \label{tab:molecular_property_prediction} 
    \vspace{.1in}
    \resizebox{\textwidth}{!}{\begin{tabular}{l|ccc|ccccccc}
        \toprule
        Dataset & ESOL & FREESOLV & LIPO & BACE & BBBP & CLINTOX & HIV & SIDER & TOX21 & TOXCAST \\
        Metric & RMSE($\downarrow$) & RMSE($\downarrow$) & RMSE($\downarrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) \\
        \midrule
        \textsc{GCN} & 0.9229{\scriptsize $\pm$0.0284} & 2.0218{\scriptsize $\pm$0.0721} & 0.7786{\scriptsize $\pm$0.0122} & \bf 79.68{\scriptsize $\pm$1.44} & 67.50{\scriptsize $\pm$0.88} & \bf 88.47{\scriptsize $\pm$1.21} & 76.27{\scriptsize $\pm$1.05} & 62.72{\scriptsize $\pm$0.70} & 75.82{\scriptsize $\pm$0.31} & 63.25{\scriptsize $\pm$0.58}\\
        \textsc{GAT} & 0.9822{\scriptsize $\pm$0.0924} & 2.1375{\scriptsize $\pm$0.0759} & 0.7629{\scriptsize $\pm$0.0202} & 77.23{\scriptsize $\pm$1.94} & 68.36{\scriptsize $\pm$0.87} & 84.24{\scriptsize $\pm$1.44} & 73.65{\scriptsize $\pm$1.91} & 58.54{\scriptsize $\pm$2.03} & 75.16{\scriptsize $\pm$0.92} & 62.24{\scriptsize $\pm$1.25}\\
        \textsc{SAGE} & \bf 0.8389{\scriptsize $\pm$0.0122} & 2.1231{\scriptsize $\pm$0.0514} & \bf 0.7086{\scriptsize $\pm$0.0087} & 76.25{\scriptsize $\pm$1.49} & 66.73{\scriptsize $\pm$0.86} & 86.33{\scriptsize $\pm$2.12} & 74.81{\scriptsize $\pm$1.43} & \bf 64.06{\scriptsize $\pm$0.93} & \bf 75.96{\scriptsize $\pm$0.50} & \bf 65.56{\scriptsize $\pm$0.56} \\
        \textsc{SGC} & 0.9784{\scriptsize $\pm$0.0148} & \bf 2.0195{\scriptsize $\pm$0.0625} & 0.7838{\scriptsize $\pm$0.0096} & 75.01{\scriptsize $\pm$1.59} & 67.22{\scriptsize $\pm$0.74} & 85.66{\scriptsize $\pm$1.33} & 73.97{\scriptsize $\pm$1.20} & 62.42{\scriptsize $\pm$1.16} & 74.23{\scriptsize $\pm$0.52} & 63.60{\scriptsize $\pm$0.54} \\
        \textsc{TokenGT} & 0.8766{\scriptsize $\pm$0.0210} & 2.0783{\scriptsize $\pm$0.1061} & 0.8020{\scriptsize $\pm$0.0127} & 79.03{\scriptsize $\pm$1.56} & 68.00{\scriptsize $\pm$0.87} &  &  & 61.41{\scriptsize $\pm$1.32} & 75.07{\scriptsize $\pm$0.38} & \\
        \midrule
        \textsc{HGCN} & 0.9820{\scriptsize $\pm$0.0215} & 2.3192{\scriptsize $\pm$0.0990} & 0.7344{\scriptsize $\pm$0.0089} & 76.61{\scriptsize $\pm$1.65} & 66.16{\scriptsize $\pm$1.40} & 80.62{\scriptsize $\pm$2.27} & \bf 76.57{\scriptsize $\pm$0.90} & \texttt{NaN} & 75.71{\scriptsize $\pm$0.44} & \texttt{NaN}\\
        \textsc{HGNN} & 1.0049{\scriptsize $\pm$0.0378} & 2.3245{\scriptsize $\pm$0.1527} & 0.7422{\scriptsize $\pm$0.0096} & 74.56{\scriptsize $\pm$2.96} & \bf 69.54{\scriptsize $\pm$0.99} & 81.16{\scriptsize $\pm$3.41} & 74.68{\scriptsize $\pm$1.00} & 57.84{\scriptsize $\pm$0.82} & 75.40{\scriptsize $\pm$0.33} & 64.00{\scriptsize $\pm$0.36} \\
        \textsc{HAT} & 1.4327{\scriptsize $\pm$0.0414} & 2.6332{\scriptsize $\pm$0.1086} & 0.8313{\scriptsize $\pm$0.0123} & 74.71{\scriptsize $\pm$2.31} & 65.97{\scriptsize $\pm$1.36} & 72.57{\scriptsize $\pm$2.17} & 71.56{\scriptsize $\pm$0.98} & 57.96{\scriptsize $\pm$1.74} & 73.16{\scriptsize $\pm$0.50} & 62.49{\scriptsize $\pm$0.62} \\
        \midrule
        \textsc{$\kappa$-GCN} & 1.2207{\scriptsize $\pm$0.1883} & 2.9561{\scriptsize $\pm$0.2671} & 0.8681{\scriptsize $\pm$0.0340} & 72.10{\scriptsize $\pm$2.49} & 61.98{\scriptsize $\pm$2.58} & 51.07{\scriptsize $\pm$4.94} & 72.59{\scriptsize $\pm$1.19} & 52.86{\scriptsize $\pm$1.29} & 70.10{\scriptsize $\pm$0.48} & 60.12{\scriptsize $\pm$0.97} \\
        \textsc{$\mathcal{Q}$-GCN} & 0.9756{\scriptsize $\pm$0.0301} & 2.3538{\scriptsize $\pm$0.0590} & 0.7465{\scriptsize $\pm$0.0115} & 77.15{\scriptsize $\pm$1.86} & 66.33{\scriptsize $\pm$1.16} & 79.45{\scriptsize $\pm$2.55} &  & 59.77{\scriptsize $\pm$1.33} & 75.10{\scriptsize $\pm$0.43} & 63.85{\scriptsize $\pm$0.44}\\
        \midrule
        \textsc{\modelname{}} &  &  &  &  &  &  &  &  &  & \\
        \bottomrule
    \end{tabular}
    }
\end{table}



==> tables/rebuttal_GR_runtime.tex <==
\begin{table}[!ht]
    \centering
    \caption{Average runtime (in ms) during inference for each method across datasets. Each result is from averaging over 20 different runs.}\label{fig:rebuttal_computational_cost}
    \vspace{5pt}
    \resizebox{.6\textwidth}{!}{\begin{tabular}{cc|cccc}
    \toprule
    Model & Dimension & Web-Edu & Power & Facebook & Bio-Worm \\
    \midrule
    \multirow{4}{*}{TokenGT} & 2 &  &  &  &  \\
    & 4 &  &  &  &  \\
    & 8 &  &  &  &  \\
    & 16 &  &  &  &  \\
    \midrule
    \multirow{4}{*}{FPS-T (ours)} & 2 &  &  &  &  \\
    & 4 &  &  &  &  \\
    & 8 &  &  &  &  \\
    & 16 &  &  &  &  \\
    \bottomrule
    \end{tabular}
    }
    %\vspace{-20px}
\end{table}


==> tables/rebuttal_runtime.tex <==
\begin{table}[!ht]
    \centering
    \caption{Average runtime (in ms) during inference for each method across datasets. Each result is from averaging over 20 different runs.}\label{fig:rebuttal_computational_cost}
    \vspace{5pt}
    \resizebox{\textwidth}{!}{\begin{tabular}{l|cccc|cccc|cccc}
    \toprule
    Dataset & Web-Edu & Power & Facebook & Bio-Worm & Texas & Cornell & Wisconsin & Actor & Airport & Citeseer & Pubmed & Cora \\
    \midrule
    \# nodes & 3,031 & 4,941 & 4,039 & 2,274 & 183 & 183 & 251 & 7,600 & 3,188 & 3,327 & 19,717 & 2,708 \\
    \# edges & 6,474 & 6,594 & 78.328 & 88,234 & 325 & 298 & 515 & 30,019 & 18,631 & 4,732 & 44,338 & 5,429 \\
    \midrule
    GCN & 0.71 & 2.54 & 2.71 & 1.45 &  &  &  &  &  &  &  &  \\
    GAT & 7.90 & 7.35 & 11.24 & 7.86 &  &  &  &  &  &  &  &  \\
    SAGE & 10.90 & 9.13 & 22.20 & 7.66 &  &  &  &  &  &  &  &  \\
    SGC & 1.11 & 2.35 & 3.12 & 2.02 &  &  &  &  &  &  &  &  \\
    TokenGT & 10.10 & 8.93 & 57.09 & 50.28 &  &  &  &  &  &  &  &  \\
    \midrule
    HGCN & 8.55 & 10.64 & 9.50 & 9.06 &  &  &  &  &  &  &  &  \\
    HGNN & 5.90 & 6.51 & 9.57 & 9.59 &  &  &  &  &  &  &  &  \\
    HAT & 17.50 & 20.11 & 20.11 & 16.15 &  &  &  &  &  &  &  &  \\
    \midrule
    $\kappa$-GCN & 7.91 & 10.68 & 8.84 & 8.03 &  &  &  &  &  &  &  &  \\
    $\mathcal{Q}$-GCN & 72.09 & 75.36 & 74.62 & 72.42 &  &  &  &  &  &  &  &  \\
    \midrule
    \modelname{} (ours) & 22.72 & 21.64 & 70.94 & 66.44 &  &  &  &  &  &  &  &  \\
    \bottomrule
    \end{tabular}
    }
    %\vspace{-20px}
\end{table}


==> tables/rebuttal_synthetic.tex <==
\begin{table}[!h]
    \centering
    \caption{Average distortion from running graph reconstruction on four synthetic geometric graphs (lower is better). FPS-T consistently outperforms its Euclidean counterpart, with learnable curvatures converging to signs that align with the input geometry despite being initialized at zero. For instance, FPS-T learns one positive and one negative curvature when trained on reconstructing a Ring of Trees.}\label{fig:synthetic}
    \vspace{5pt}
    \resizebox{.85\textwidth}{!}{\begin{tabular}{cc|cccc}
    \toprule
    Model & Space & Tree & Sphere & Torus & Ring of Trees \\
    \midrule
    \multirow{2}{*}{TokenGT} & $\E^{10}$ & 0.04363 & 0.04023 & 0.07172 & 0.05553 \\
    & $\E^5 \times \E^5$ & 0.04357 & 0.04139 & 0.07167 & 0.05546\\
    \midrule
    \multirow{2}{*}{FPS-T (ours)} & $\mathfrak{st}_{\kappa_1}^{10}$ & \bf 0.00072 & \bf 0.02176 & 0.06415 & 0.03393\\
    & $\mathfrak{st}^5_{\kappa_1} \times \mathfrak{st}^5_{\kappa_2}$ & 0.00105 & 0.02206 & \bf 0.06135 & \bf 0.01630\\
    \midrule
    \multicolumn{2}{c|}{Best FPS-T curvatures} & $(-1.219)$ & $(+0.0629)$ & $(+1.308, +0.2153)$ & $(+0.3241, -3.314)$ \\
    \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/stereographic_nn.tex <==
\begin{table}[t!]
    \centering
    \caption{TODO.} \label{tab:stereographic_ops} 
    \vspace{.1in}
    \begin{tabular}{l l c}
        \toprule
        Neural Networks & \multicolumn{1}{c}{$\kappa \in \R$} & $\kappa \rightarrow 0$ \\
        \midrule
        Linear & & \\
        Activation & & \\
        Logits & & \\
        \bottomrule
    \end{tabular}
\end{table}

